Two-Layer Model Predictive Battery Thermal and Energy Management Optimization for Connected and Automated Electric Vehicles

Future vehicles are expected to be able to exploit increasingly the connected driving environment for efficient, comfortable, and safe driving. Given relatively slow dynamics associated with the state of charge and temperature response in electrified vehicles with large batteries, a long prediction/planning horizon is needed to achieve improved energy efficiency benefits. In this paper, we develop a two-layer Model Predictive Control (MPC) strategy for battery thermal and energy management of electric vehicle (EV), aiming at improving fuel economy through real-time prediction and optimization. In the first layer, the long-term traffic flow information and an approximate model reflective of the relatively slow battery temperature dynamics are leveraged to minimize energy consumption required for battery cooling while maintaining the battery temperature within the desired operating range. In the second layer, the scheduled battery thermal and state of charge (SOC) trajectories planned to achieve long-term battery energy-optimal thermal behavior are used as the reference over a short horizon to regulate the battery temperature. Additionally, an intelligent online constraint handling (IOCH) algorithm is developed to compensate for the mismatch between the actual and predicted driving conditions and reduce the chance for battery temperature constraint violation. The simulation results show that, depending on the driving cycle, the proposed two-layer MPC is able to save 2.8-7.9% of the battery energy compared to the traditional rule-based controller in connected and automated vehicle (CAV) operation scenario. Moreover, as compared to a single layer MPC with a long horizon, the two-layer structure of the proposed MPC solution reduces significantly the computing effort without compromising the performance.

==> ACC2018Ref <==
@article{bauer2014thermal,
  title={{Thermal and Energy Battery Management Optimization in Electric Vehicles Using Pontryagin's Maximum Principle}},
  author={Bauer, S. and Suchaneck, A. and Le{\'o}n, F.},
  journal={Journal of Power Sources},
  volume={246},
  pages={808--818},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{masoudi2017mpc,
  title={{MPC-Based Battery Thermal Management Controller for Plug-in Hybrid Electric vehicles}},
  author={Masoudi, Y. and Azad, N.},
  booktitle={American Control Conference},
  pages={4365--4370},
  year={2017}
}

@article{yuksel2012development,
title={{Development of a simulation model to analyze the effect of thermal management on battery life}},
author={Yuksel, T. and Michalek, J.},
Note={{SAE Technical Paper 2012-01-0671}},
year={2012}
}

@inproceedings{lofberg2004yalmip,
  title={{YALMIP: A Toolbox for Modeling and Optimization in MATLAB}},
  author={Lofberg, J.},
  booktitle={2004 IEEE Int. Symp. on Computer Aided Control Sys. Design},
year={2004},
note={New Orleans, LA, USA},
}

@article{wachter2006implementation,
  title={{On the Implementation of an Interior-Point Filter Line-Search Algorithm for Large-Scale Nonlinear Programming}},
  author={W{\"a}chter, A. and Biegler, L.},
  journal={Mathematical Programming},
  volume={106},
  number={1},
  pages={25--57},
  year={2006},
  publisher={Springer}
}

@article{zhang2011charge,
  title={{Charge-Depleting Control Strategies and Fuel Optimization of Blended-Mode Plug-in Hybrid Electric Vehicles}},
  author={Zhang, B. and Mi, C. and Zhang, M.},
  journal={IEEE Trans. on VT},
  volume={60},
  number={4},
  pages={1516--1525},
  year={2011},
  publisher={IEEE}
}

@article{zhang2012analytical,
  title={{Analytical Approach for the Power Management of Blended-Mode Plug-in Hybrid Electric Vehicles}},
  author={Zhang, M. and Yang, Y. and Mi, C.},
  journal={IEEE Trans. on Veh. Technology},
  volume={61},
  number={4},
  pages={1554--1566},
  year={2012},
  publisher={IEEE}
}

@article{lim2017distance,
  title={{Distance-Based Ecological Driving Scheme Using a Two-Stage Hierarchy for Long-Term Optimization and Short-Term Adaptation}},
  author={Lim, H. and Su, W. and Mi, C.},
  journal={IEEE Trans. on Vehicular Technology},
  volume={66},
  number={3},
  pages={1940--1949},
  year={2017},
  publisher={IEEE}
}

@article{halbach2010model,
  title={{Model Architecture, Methods, and Interfaces for Efficient Math-Based Design and Simulation of Automotive Control Systems}},
  author={Halbach, S. and Sharer, P. and Pagerit, S. and Rousseau, A. and Folkerts, C.},
Note={{SAE Technical Paper 2010-01-0241}},
year={2010}
}


@article{zolot2002thermal,
  title={{Thermal Evaluation of Toyota Prius Battery Pack}},
  author={Zolot, M. and Pesaran, A. and Mihalic, M.},
Note={{SAE Technical Paper 2002-01-1962}},
year={2002}
}



@inproceedings{sun2015integrating,
  title={{Integrating traffic velocity data into predictive energy management of plug-in hybrid electric vehicles}},
  author={Sun, C. and Sun, F. and Hu, X. and Hedrick, J. and Moura, S.},
  booktitle={ACC},
  year={2015},
  note={Chicago, IL, USA}
}

@article{lefort2013hierarchical,
  title={{Hierarchical Control Method Applied to Energy Management of a Residential House}},
  author={Lefort, A. and Bourdais, R. and Ansanay-Alex, G. and Gu{\'e}guen, H.},
  journal={Energy and Buildings},
  volume={64},
  pages={53--61},
  year={2013},
  publisher={Elsevier}
}


@article{herrera2010evaluation,
  title={{Evaluation of Traffic Data Obtained via GPS-Enabled Mobile Phones: The Mobile Century field experiment}},
  author={Herrera, J. and Work, D. and Herring, R. and Ban, X. and Jacobson, Q. and Bayen, A.},
  journal={Transportation Research Part C: Emerging Technologies},
  volume={18},
  number={4},
  pages={568--583},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{masoudi2015battery,
  title={{Battery Thermal Management of Electric Vehicles: An Optimal Control Approach}},
  author={Masoudi, Y. and Mozaffari, A. and Azad, N.},
  booktitle={ASME Dynamic Systems and Control Conf.},
 year={2015},
  note={Columbus, OH, USA}
}

@inproceedings{kim2014real,
  title={{Real-Time Battery Thermal Management for Electric Vehicles}},
  author={Kim, E. and Shin, K. and Lee, J.},
  booktitle={ACM/IEEE 5th Int. Conference on Cyber-Physical Systems},
  year={2014},
  note={Berlin, Germany}
}

@article{cominesi2018two,
  title={{A Two-Layer Stochastic Model Predictive Control Scheme for Microgrids}},
  author={Cominesi, S. and Farina, M. and Giulioni, L. and Picasso, B. and Scattolini, R.},
  journal={IEEE Trans. on Control systems Technology},
  volume={26},
  number={1},
  pages={1--13},
  year={2018},
  publisher={IEEE}
}

@article{farina2018hierarchical,
  title={{A Hierarchical Multi-Rate MPC Scheme for Interconnected Systems}},
  author={Farina, M. and Zhang, X. and Scattolini, R.},
  journal={Automatica},
  volume={90},
  pages={38--46},
  year={2018},
  publisher={Elsevier}
}


@article{guanetti2018control,
  title={{Control of Connected and Automated Vehicles: State of the Art and Future Challenges}},
  author={Guanetti, J. and Kim, Y. and Borrelli, F.},
  journal={Annual Reviews in Control},
  volume={45},
  pages={18--40}
  year={2018},
  publisher={Elsevier}
}

@article{neubauer2014thru,
  title={{Thru-life Impacts of Driver Aggression, Climate, Cabin Thermal Management, and Battery Thermal Management on Battery Electric Vehicle Utility}},
  author={Neubauer, J. and Wood, E.},
  journal={Journal of Power Sources},
  volume={259},
  pages={262--275},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{hwang2018,
  title={{Model Predictive Climate Control of Connected and Automated Vehicles for Improved Energy Efficiency}},
  author={Wang, H. and Kolmanovsky, I. and Amini, M. and Sun, J.},
  booktitle={ACC},
  year={2018},
note={{Milwaukee, WI, USA}}
}
